Phoenix: An Epidemic Approach to Time Reconstruction

Harsh deployment environments and uncertain run-time conditions create numerous challenges for postmortem time reconstruction methods. For example, motes often reboot and thus lose their clock state, considering that the majority of mote platforms lack a real-time clock. While existing time reconstruction methods for long-term data gathering networks rely on a persistent basestation for assigning global timestamps to measurements, the basestation may be unavailable due to hardware and software faults. We present Phoenix, a novel offline algorithm for reconstructing global timestamps that is robust to frequent mote reboots and does not require a persistent global time source. This independence sets Phoenix apart from the majority of time reconstruction algorithms which assume that such a source is always available. Motes in Phoenix exchange their time-related state with their neighbors, establishing a chain of transitive temporal relationships to one or more motes with references to the global time. These relationships allow Phoenix to reconstruct the measurement timeline for each mote. Results from simulations and a deployment indicate that Phoenix can achieve timing accuracy up to 6 ppm for 99% of the collected measurements. Phoenix is able to maintain this performance for periods that last for months without a persistent global time source. To achieve this level of performance for the targeted environmental monitoring application, Phoenix requires an additional space overhead of 4% and an additional duty cycle of 0.2%.

==> Makefile <==
all: topo.eps seglen.eps reboot_bv.eps badbeta.eps fits.eps \
	nobs_ppm.eps wake_dloss.eps bad_anchors.eps \
	evict_space.eps evict_dc.eps evict_dloss.eps density_dloss.eps \
	olin_alpha.eps koala_phoenix.eps \
	path.eps

%.eps: %.R
	R --no-save < $<

==> chapter5.tex <==
\chapter{Time Reconstruction II - Phoenix}
\label{chap:phoenix}

One of the big take aways from Sundial was to collect enough number of
(local,global) reference points so that all the segments can be assigned a
global timestamps. Employing a persistent basestation and performing regular
downloads seemed like a reasonable way to achieve this. In the Cub Hill
deployment, we put this to practise and it worked out well for the vast
majority of segments. One of the things we overlooked was that the basestation
is susceptible to failures and performing regular downloads may not always be
possible due to power constraints.

In this chapter, I will present the reasons behind why we needed to design a
new time reconstruction methodology that does not require a persistent global
clock source and can tolerate random mote resets. I'll present a summary of
Phoenix at this point and details of the method in the rest of the chapter. 

Motes in Phoenix exchange their time-related state with their neighbors,
establishing a chain of transitive temporal relationships to one or more motes
with references to the global time. These relationships allow Phoenix to
reconstruct the measurement timeline for each mote. Results from simulations
and a deployment indicate that Phoenix can achieve timing accuracy up to 6 ppm
for 99\% of the collected measurements. Phoenix is able to maintain this
performance for periods that last for months without a persistent global time
source. To achieve this level of performance for the targeted environmental
monitoring application, Phoenix requires an additional space overhead of 4\%
and an additional duty cycle of 0.2\%.

\input{phoenix/intro}

\input{phoenix/mot}

\input{phoenix/soln}

\input{phoenix/results}

\input{phoenix/relwork}

\input{phoenix/concl}

\noindent


==> impact.tex <==
\section{Impact}
\label{sec:impact}

We evaluate the impact of mote reboots on the $C$ deployment using
our existing time reconstruction methodology. 

When a
mote is contacted for a download, the basestation records an
anchor point. i.e. it records the mote's current local clock and the
basestation's global clock. Motes that are poorly connected to
the basestation can remain out of contact with the basestation for
several download rounds before they can transfer their outstanding data.
When motes reboot at a rate faster than the frequency with which they
contact the basestation, there exist periods which lack enough information
to accurately recover the timestamps.

Upon acquiring the anchor points, the measurements are converted from
their local clock to the global clock using the Robust Global
Timestamp Reconstruction algorithm (RGTR, \cite{SUN+EWSN+09}).  We
note that, in order to estimate the fit parameters ($\alpha$, $\beta$)
for the segments, RGTR requires at least 2 anchor points. If we 
assume that $\alpha$ is stable per mote for small segments. Using this
assumption, at least one anchor point is needed to estimate the
$\beta$ for any given segment, provided that $\alpha$ has been
estimated accurately for the mote.


\begin{figure}[t]
\centering 
\subfigure[The fraction of measurements that were assigned timestamps]
{\label{sfig:recon} \includegraphics[scale=0.7]{./graphs/fits.eps}}
\subfigure[An example of estimating $\beta$ incorrectly when
using approximate methods.]
{\label{sfig:appx} \includegraphics[scale=0.7]{./graphs/badbeta.eps}}
  \caption{Impact due to existing time reconstruction methodology}
  \label{fig:impact}
\end{figure}


\subsection{Quantifying the Impact}
Figure \ref{sfig:recon} demonstrates the impact of mote reboots on 
time reconstruction for the $C$ deployment.  In period A, the samples 
collected falls because some notes were freezing.  At B, the watchdog 
timer fix was added, and the samples collected returns to near the 
expected level. However, due to the increased frequency of reboots, a 
larger portion of the samples couldn't be timestamped (exacerbated by 
the absence of the base station during period C.}


For segments where no anchor points were collected, we assumed that
node reboots are instantaneous. 
This assumption
does not always hold, and leads to a small fraction of misaligned
measurements. An example of this is shown in Figure
\ref{sfig:appx}. Box 220 was in-sync with the other boxes till
June 22, 2009. It then rebooted multiple times and could not reach the
basestation during these periods. The approximate
timestamp approach resulted in a bad estimate of the $\beta$ parameter
for those segments. It is clear that the timestamps for the period
after the reboot are shifted. A cross-correlation between the PAR data
(or another suitable modality) from this box and from the nearby ones can
help in recovering this shift. \dc{could cut out final sentence}

